Regular decompositions of finite root systems and simple Lie algebras

Let $\mathfrak{g}$ be a finite-dimensional simple Lie algebra over an algebraically closed field of characteristic 0. In this paper we classify all regular decompositions of $\mathfrak{g}$ and its irreducible root system $\Delta$. A regular decomposition is a decomposition $\mathfrak{g} = \mathfrak{g}_1 \oplus \dots \oplus \mathfrak{g}_m$, where each $\mathfrak{g}_i$ and $\mathfrak{g}_i \oplus \mathfrak{g}_j$ are regular subalgebras. Such a decomposition induces a partition of the corresponding root system, i.e. $\Delta = \Delta_1 \sqcup \dots \sqcup \Delta_m$, such that all $\Delta_i$ and $\Delta_i \sqcup \Delta_j$ are closed. Partitions of $\Delta$ with $m=2$ were known before. In this paper we prove that the case $m \ge 3$ is possible only for systems of type $A_n$ and describe all such partitions in terms of $m$-partitions of $(n+1)$. These results are then extended to a classification of regular decompositions of $\mathfrak{g}$.

==> settings.tex <==
%% For formatting the tables
\usepackage{array}

%% Geometry of the page
\RequirePackage[margin=3.5cm]{geometry}

%% Pictures and figures
\usepackage{graphicx}
\usepackage{svg}
\usepackage{float} % to use H option
\usepackage{pdfpages} % to insert pdfs

%% Font encodings
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}

\usepackage{titlesec}
\titleformat{\section}
  {\Large\sc}
  {\thesection}{1em}{}
\titleformat{\subsection}
  {\large\sc}
  {\thesubsection}{1em}{}


    

%% Bibliography
\usepackage[
backend=bibtex,
style=numeric,
maxbibnames=99,
maxcitenames = 99
]{biblatex}
\addbibresource{bibliography.bib}


%%%%%%%%%%%%%%% MATH (and references) %%%%%%%%%%%%%%%
%% Math packages
\usepackage{amsmath, amsthm, amssymb}
\usepackage{mathtools}
\usepackage{relsize} % to make mathsymbols larger

%% References
\usepackage{nameref}
\usepackage{hyperref}
% \hypersetup{colorlinks,
%   linkcolor=ThesisDarkBlue,
%   citecolor=ThesisPurple,
%   urlcolor=ThesisDarkBlue,
%   filecolor=ThesisDarkBlue}
\usepackage[capitalise, nameinlink]{cleveref} % has to be added after amsmath
\newcommand{\crefrangeconjunction}{--}

%% QED symbol = black square
\renewcommand{\qedsymbol}{\ensuremath{\blacksquare}}

%% Mathfrak
\newcommand{\fg}[0]{\mathfrak{g}}
\newcommand{\fp}[0]{\mathfrak{p}}
\newcommand{\fs}[0]{\mathfrak{s}}
\newcommand{\fn}{\mathfrak{n}}
\newcommand{\fh}{\mathfrak{h}}
\newcommand{\fb}[0]{\mathfrak{b}}
\newcommand{\fT}{\mathfrak{T}}
\newcommand{\fD}{\mathfrak{D}}

%% Killing form
\newcommand{\kf}{\kappa}

%% Mathbb
\newcommand{\bC}[0]{\mathbb{C}}
\newcommand{\bN}[0]{\mathbb{N}}
\newcommand{\bZ}[0]{\mathbb{Z}}
\newcommand{\bR}[0]{\mathbb{R}}

%% Operators
\newcommand{\add}{\dotplus}
\newcommand{\ot}{\otimes}
\newcommand{\op}{\oplus}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\Aut}{Aut}
\DeclareMathOperator{\colim}{colim}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\ad}{ad}

%%
\renewcommand{\ge}{\geqslant}
\renewcommand{\le}{\leqslant}

%%%%%%%%%%% ENVIRONMENTS %%%%%%%%%%%%%%%%
\newtheorem{thm}{Theorem}[section]
\theoremstyle{plain}

\newtheorem{corollary}[thm]{Corollary}
\newtheorem{lemma}[thm]{Lemma}
\newtheorem{proposition}[thm]{Proposition}
\newtheorem{theorem}[thm]{Theorem}
\newtheorem{conjecture}[thm]{Conjecture}


% Environments for main results in the introduction 

\newtheorem{theoremcounter}{theoremcounter}[section]
\newtheorem{maintheoremcounter}{maintheoremcounter}

\newtheorem{maincorollary}[maintheoremcounter]{Corollary}

\newtheorem{maintheorem}[maintheoremcounter]{Theorem}
\renewcommand{\themaintheoremcounter}{\Alph{maintheoremcounter}}

% Definitions

\theoremstyle{definition}
\newtheorem{definitionx}[thm]{Definition}
\newenvironment{definition}
  {\pushQED{\qed}\renewcommand{\qedsymbol}{$\lozenge$}\definitionx}
 {\popQED\enddefinitionx}

% Example/Remark style
\newtheoremstyle{example_style}
  {5pt} % Space above
  {5pt} % Space below
  {} % Body font
  {} % Indent amount
  {\itshape} % Theorem head font
  {.} % Punctuation after theorem head
  {10pt} % Space after theorem head
  {} % Theorem head spec (can be left empty, meaning `normal')

\theoremstyle{example_style}
% examplex is wrapped into example, which just adds lozenge at the end
\newtheorem{examplex}[thm]{Example}
\newenvironment{example}
  {\pushQED{\qed}\renewcommand{\qedsymbol}{$\lozenge$}\examplex}
  {\popQED\endexamplex}

\crefname{examplex}{Example}{Examples} % Name for cleverref

% Similarly with remark
\newtheorem{remarkx}[thm]{Remark}
\newenvironment{remark}
  {\pushQED{\qed}\renewcommand{\qedsymbol}{$\lozenge$}\remarkx}
 {\popQED\endremarkx}


%%% FONT %%%%%%
\usepackage{newpxtext,newpxmath}


%%%%% TIKZ-CD %%%%%%%%%%%%%%
\usepackage{tikz-cd}

